A Radial Basis Function (RBF)-Finite Difference (FD) Method for Diffusion and Reaction-Diffusion Equations on Surfaces

In this paper, we present a method based on Radial Basis Function (RBF)-generated Finite Differences (FD) for numerically solving diffusion and reaction-diffusion equations (PDEs) on closed surfaces embedded in $\mathbb{R}^d$. Our method uses a method-of-lines formulation, in which surface derivatives that appear in the PDEs are approximated locally using RBF interpolation. The method requires only scattered nodes representing the surface and normal vectors at those scattered nodes. All computations use only extrinsic coordinates, thereby avoiding coordinate distortions and singularities. We also present an optimization procedure that allows for the stabilization of the discrete differential operators generated by our RBF-FD method by selecting shape parameters for each stencil that correspond to a global target condition number. We show the convergence of our method on two surfaces for different stencil sizes, and present applications to nonlinear PDEs simulated both on implicit/parametric surfaces and more general surfaces represented by point clouds.

==> EpsHeur.tex <==
\section{A Heuristic for $\ep$}
\label{sec:results3}

In this section, we present a statistical model for generating the shape parameter $\ep_k$ on a surface stencil $P_k$, given the minimum width $h^{min}_k$ between any two points on $P_k$ and the desired condition number $\kappa_T$ of the RBF interpolation matrix $A_{P_k}$ on that stencil.

As was mentioned in Section \ref{sec:stability}, the exact shape parameter $\ep_k$ for a given stencil $P_k$ on the surface is computed by determining the zero of the function presented in that section. However, depending on the target condition number $\kappa_T$, a solver may take several iterations to find the interval in which the zero crossing of the function lies and then several more iterations to compute the value of the zero itself.

Given a set of $N$ nodes, $X$, on a surface, our goal is therefore to present a procedure by which one can determine an approximation to the shape parameter $\ep_k$ for all $N$ stencils $P_k$ on that surface. We envision using this approximation as a good starting guess for the solver, thereby reducing the number of iterations taken by the solver to compute the exact shape parameter $\ep_k$; indeed, we adopt this approach in our own tests. Alternatively, one could use the approximate shape parameter $\hat{\ep}_k$ in place of the exact shape parameter, though we do not explore that approach in this work.

In generating our statistical model, we bear in mind that the condition $\ep_k>0$ must be true. We also know that the inputs to the model are always positive, {\em i.e.,} $h^{min}_k > 0$ and $\kappa_T > 0$. Since $\kappa_T$ is a very large number and $0 < h^{min}_k < 1$, it is useful to use the logarithm of $\kappa_T$, $l_{\kappa} = \log(\kappa_T)$, as the input to the model instead of $\kappa_T$ itself. Also, in general, we expect $\ep_k \propto \frac{1}{h^{min}_k}$. So, for convenience, let $r_k = \frac{1}{h^{min}_k}$.  Given these conditions, we now seek a relationship of the form
%
\begin{align}
\log(\ep_k) \approx \log(\hat{\ep}_k) = s\lf(r_k, l_{\kappa}\rt),
\end{align}
%
where $s$ is some function of the inputs to the model; this formulation ensures that the resulting $\hat{\ep}_k$ is always positive. We determine the function $s$ as follows:

\begin{enumerate}
\item We record the exact value of $\ep_k$ for each stencil $P_k, k=1,\ldots,N$ on the sphere, for $610 \leq N \leq 10000$ icosahedral points.Since $h^{min}_k \propto \frac{1}{\sqrt{N}}$, this gives us an idea of how $\ep_k$ is varying with $h^{min}_k$.


\item We repeat the above step for different values of $\kappa_T$, {\em i.e.,} we set $\kappa_T = 10^4$, $10^6$, $10^8$, $10^{10}$, $10^{12}$, $10^{14}$, $k=1,...,N$, and collect the corresponding $\ep_k$ and $h^{min}_k$ values.

\item We use simple 2D polynomial regression to determine $s(r_k,l_{\kappa})$, given the list of values of $\ep_k$, $h^{min}_k$ and $\kappa_T$.
\end{enumerate}

With this method, while there are many candidates for $s$, we find that choosing $s$ to be a bivariate cubic polynomial in $r_k$ and $l_{\kappa}$ results in the approximant with the lowest residual that also fits over 99\% of the data. We present the coefficients of this cubic polynomial in Table \ref{tab:poly}.
%
\begin{table}
\centering
\begin{tabular}{|c|c|c|}
\hline
\textbf{Powers of $r_k$} & \textbf{Powers of $l_{\kappa}$} & \textbf{Coefficients} \\ \toprule \hline
3&0&1.1012e-04 \\\hline
2&1&-7.1270e-05 \\\hline
2&0&-0.0071 \\\hline
1&2&7.0963e-05 \\\hline
1&1&0.0011 \\\hline
1&0&0.2112 \\\hline
0&3&-7.9245e-05 \\\hline
0&2&0.0028 \\\hline
0&1&-0.2005 \\\hline
0&0&1.1472 \\\hline
\end{tabular}
\caption{The above table shows the coefficients of all the terms of the polynomial function $s(r_k,l_{\kappa})$. To form the polynomial, for each row, raise each variable to the number in its column, multiply across columns, and finally add all the row products.}
\label{tab:poly}
\end{table}
%
We note that the existence of a reasonable fit to the data does not by itself indicate that this log-cubic relationship is reasonable for every point set on every manifold. However, we do envision the process by which we generated the function $s$ being useful in determining approximations to the exact shape parameter on stencils of arbitrary point sets. Though we built our polynomial function $s$ with data from icosahedral points on the sphere, we use this function to generate starting guesses on all the surfaces in the following sections.

